Human-Centric Foundation Models: Perception, Generation and Agentic Modeling

Human understanding and generation are critical for modeling digital humans and humanoid embodiments. Recently, Human-centric Foundation Models (HcFMs) inspired by the success of generalist models, such as large language and vision models, have emerged to unify diverse human-centric tasks into a single framework, surpassing traditional task-specific approaches. In this survey, we present a comprehensive overview of HcFMs by proposing a taxonomy that categorizes current approaches into four groups: (1) Human-centric Perception Foundation Models that capture fine-grained features for multi-modal 2D and 3D understanding. (2) Human-centric AIGC Foundation Models that generate high-fidelity, diverse human-related content. (3) Unified Perception and Generation Models that integrate these capabilities to enhance both human understanding and synthesis. (4) Human-centric Agentic Foundation Models that extend beyond perception and generation to learn human-like intelligence and interactive behaviors for humanoid embodied tasks. We review state-of-the-art techniques, discuss emerging challenges and future research directions. This survey aims to serve as a roadmap for researchers and practitioners working towards more robust, versatile, and intelligent digital human and embodiments modeling.

==> sections/04_AIGC_papers.tex <==
% A foundation model is a machine learning or deep learning model that is trained on *Broad Data* such that it can be applied across a *Wide Range of Use Cases*.

% Image Generation

% HumanSD: A Native Skeleton-Guided Diffusion Model for Human Image Generation
% Broad Data: three large-scale human-centric datasets containing high-quality images and the corresponding 2D skeletal information and text descriptions: GHI (1M), LAION-Human (1M), and Human-Art (50K).
% Wide Use Cases: multi-scenario human-centric image generation with precise pose control.


% HyperHuman: Hyper-Realistic Human Generation with Latent Structural Diffusion
% Broad Data: 340M images with comprehensive annotations like human pose, depth, and surface-normal.
% Wide Use Cases: simultaneously generates the coarse RGB, depth, normal, and high-resolution images conditioned on text and skeleton. Both photo-realistic images and stylistic renderings can be created.

% CosmicMan: A Text-to-Image Foundation Model for Humans
% Broad Data: 6 Million high-quality real-world human images in a mean resolution of 1488×1255, and attached with precise text annotations deriving from 115 Million attributes in diverse granularities.
% Wide Use Cases: human-centric content generation tasks: Text to Image, 2D Human Editing, 3D Human Reconstruction



% Video Generation

% Human4DiT: 360-degree Human Video Generation with 4D Diffusion Transformer
% Broad Data: we collect a new multi-dimensional dataset comprises human images, videos, multiview videos, 3D data, as well as a small amount of 4D data spanning different viewpoints and time steps. It contains 5k 3D human scans capture by camera rigs, 10k videos from YouTube/Bilibili, and 100 animatable human models from artists.
% Wide Use Cases: monocular video generation, 360-degree video generation, 3D static video generation, multiview video generation

% Body of Her: A Preliminary Study on End-to-End Humanoid Agent
% SOLAMI: Social Vision-Language-Action Modeling for Immersive Interaction with 3D Autonomous Characters

% Applications
% DynVideo-E: Harnessing Dynamic NeRF for Large-Scale Motion- and View-Change Human-Centric Video Editing



% Motion Generation

% Large Motion Model for Unified Multi-Modal Motion Generation
% Broad Data: We consolidate datasets with different modalities, formats and tasks into a comprehensive yet unified motion generation dataset, MotionVerse, comprising 10 tasks, 16 datasets, a total of 320k sequences, and 100 million frames.
% Wide Use Cases: text to motion, action to motion, speech to gesture, music to dance, motion prediction

% Exploring Vision Transformers for 3D Human Motion-Language Models with Motion Patches
% Broad Data: HumanML3D and KIT Motion-Language dataset.
% Wide Use Cases: text to motion, motion to text, cross-skeleton recognition, zero-shot motion classification, human interaction recognition

% FreeMotion: MoCap-Free Human Motion Synthesis with Multimodal Large Language Models
% Broad Data: without any motion data (?)
% Wide Use Cases: motion synthesis, style transfer, human-scene interaction, and stepping stones


% HOI


% ManiVideo: Generating Hand-Object Manipulation Video with Dexterous and Generalizable Grasping


% Paper list

% Image X GAN

% StyleGAN-Human: A Data-Centric Odyssey of Human Generation
% Text2Human: Text-Driven Controllable Human Image Generation
% UnitedHuman: Harnessing Multi-Source Data for High-Resolution Human Generation

% Image X Diffusion
% HumanDiffusion: a Coarse-to-Fine Alignment Diffusion Framework for Controllable Text-Driven Person Image Generation

==> sections/perception_foundation_papers.tex <==
%  for single human-centric task
\section{ReID foundation}
All in One Framework for Multimodal Re-Identification in the Wild

Instruct-ReID: A Multi-Purpose Person Re-Identification Task with Instructions

Instruct-ReID++: Towards Universal Purpose Instruction-Guided Person Re-identification

\section{smpl foundation}
SMPLer-X: Scaling Up Expressive Human Pose and Shape Estimation

\section{detection foundation}
When Pedestrian Detection Meets Multi-Modal Learning: Generalist Model and Benchmark Dataset

% for multiple human-centric tasks
\section{pretrain-to-finetune}
Beyond Appearance: A Semantic Controllable Self-Supervised Learning Framework for Human-Centric Visual Tasks (ssl)

Versatile Multi-Modal Pre-Training for Human-Centric Perception

HAP: Structure-Aware Masked Image Modeling for Human-Centric Perception

HumanBench: Towards General Human-Centric Perception with Projector Assisted Pretraining

Efficient Multi-modal Human-Centric Contrastive Pre-training with a Pseudo Body-Structured Prior

LIFTEDCL: LIFTING CONTRASTIVE LEARNING FOR HUMAN-CENTRIC PERCEPTION

Cross-view and Cross-pose Completion for 3D Human Understanding (ssl)

\section{unified modeling}
unihcp

hulk

motionbert

You Only Learn One Query: Learning Unified Human Query for Single-Stage Multi-Person Multi-Task Human-Centric Perception

RefHCM: A Unified Model for Referring Perceptions in Human-Centric Scenarios


